STaCK: Sentence Ordering with Temporal Commonsense Knowledge

Sentence order prediction is the task of finding the correct order of sentences in a randomly ordered document. Correctly ordering the sentences requires an understanding of coherence with respect to the chronological sequence of events described in the text. Document-level contextual understanding and commonsense knowledge centered around these events are often essential in uncovering this coherence and predicting the exact chronological order. In this paper, we introduce STaCK -- a framework based on graph neural networks and temporal commonsense knowledge to model global information and predict the relative order of sentences. Our graph network accumulates temporal evidence using knowledge of `past' and `future' and formulates sentence ordering as a constrained edge classification problem. We report results on five different datasets, and empirically show that the proposed method is naturally suitable for order prediction. The implementation of this work is publicly available at: https://github.com/declare-lab/sentence-ordering.

==> results/ablation.tex <==
\begin{table}[ht!]
 %\small
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{l|cccccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{NeurIPS}} & \multicolumn{2}{c}{\textbf{AAN}} & \multicolumn{2}{c}{\textbf{NSF}} & \multicolumn{2}{c}{\textbf{SIND}} & \multicolumn{2}{c}{\textbf{ROCStory}} \\
& $\tau$ & PMR & $\tau$ & PMR & $\tau$ & PMR & $\tau$ & PMR & $\tau$ & PMR \\
\midrule
Proposed & \textbf{0.8166} & \textbf{37.31} & \textbf{0.8556} & \textbf{54.01} & 0.6582 & 12.26 & \textbf{0.6194} & \textbf{20.79} & \textbf{0.8534} & \textbf{55.96} \\
\quad same CSK Edges: $r_p = r_f$ & 0.8146 & 37.06 & 0.8472 & 52.25 & \textbf{0.6642} & \textbf{12.41} & 0.6172 & 20.03 & 0.8470 & 54.32 \\
\quad w/o CSK Nodes, Edges & 0.8035 & 33.30 & 0.8365 & 50.10 & 0.6567 & 11.79 & 0.6154 & 19.84 & 0.8391 & 53.04 \\
% \quad w/o Global Node & & & & & & & & & & \\
\bottomrule
\end{tabular}
}
\caption{\footnotesize Ablation study w.r.t CSK components. Scores are reported at best validation $\tau$.}
\label{tab:ablation}
\end{table}


